On the complexity of Client-Waiter and Waiter-Client games

Positional games were introduced by Hales and Jewett in 1963, and their study became more popular after Erdos and Selfridge's first result on their connection to Ramsey theory and hypergraph coloring in 1973. Several conventions of these games exist, and the most popular one, Maker-Breaker was proved to be PSPACE-complete by Schaefer in 1978. The study of their complexity then stopped for decades, until 2017 when Bonnet, Jamain, and Saffidine proved that Maker-Breaker is W[1]-complete when parameterized by the number of moves. The study was then intensified when Rahman and Watson improved Schaefer's result in 2021 by proving that the PSPACE-hardness holds for 6-uniform hypergraphs. More recently, Galliot, Gravier, and Sivignon proved that computing the winner on rank 3 hypergraphs is in P. We focus here on the Client-Waiter and the Waiter-Client conventions. Both were proved to be NP-hard by Csernenszky, Martin, and Pluh\'ar in 2011, but neither completeness nor positive results were known for these conventions. In this paper, we complete the study of these conventions by proving that the former is PSPACE-complete, even restricted to 6-uniform hypergraphs, and by providing an FPT-algorithm for the latter, parameterized by the size of its largest edge. In particular, the winner of Waiter-Client can be computed in polynomial time in k-uniform hypergraphs for any fixed integer k. Finally, in search of finding the exact bound between the polynomial result and the hardness result, we focused on the complexity of rank 3 hypergraphs in the Client-Waiter convention. We provide an algorithm that runs in polynomial time with an oracle in NP.

==> Figures/domination_game_reduction.tex <==
\begin{figure}[ht]
\centering
\scalebox{1}{
\begin{tikzpicture}

\node[noeud] (x1) at (0,0){};
\node[noeud] (x2) at (1.25,0){};
\node[noeud] (x3) at (2.5,0){};
\node[noeud] (x4) at (3.75,0){};

\node[below left] at (x1) {$v_1$};
\node[below left] at (x2) {$v_2$};
\node[below left] at (x3) {$v_3$};
\node[below right] at (x4) {$v_4$};


\node[noeud] (c1) at (-0.8,-3){};
\node[noeud] (c1b) at (0.1,-3){};
\node[noeud] (c2) at (1.5,-3){};
\node[noeud] (c2b) at (2.4,-3){};
\node[noeud] (c3) at (3.8,-3){};
\node[noeud] (c3b) at (4.7,-3){};

\node[below=1pt] at (c1){$v_A^1$};
\node[below=1pt] at (c1b) {$v_A^2$};
\node[below=1pt] at (c2) {$v_B^1$};
\node[below=1pt] at (c2b) {$v_B^2$};
\node[below=1pt] at (c3) {$v_C^1$};
\node[below=1pt] at (c3b) {$v_C^2$};

\path[draw, -, bend left = 40] (x1) to (x3)  ;
\path[draw, -, bend left = 40] (x1) to (x4)  ;
\path[draw, -, bend left = 40] (x2) to (x4)  ;
\path[draw, -] (x1) to (x2)  ;
\path[draw, -] (x2) to (x3)  ;
\path[draw, -] (x3) to (x4)  ;


\draw (x1) -- (c1);
\draw (x1) -- (c1b);
\draw (x1) -- (c2);
\draw (x1) -- (c2b);
\draw (x2) -- (c1);
\draw (x2) -- (c1b);
\draw (x2) -- (c3);
\draw (x2) -- (c3b);
\draw (x3) -- (c3);
\draw (x3) -- (c3b);
\draw (x4) -- (c2);
\draw (x4) -- (c2b);
\draw (x4) -- (c3);
\draw (x4) -- (c3b);

\node[noeud] (u1) at (-5.5,-2.25){};
\node[noeud] (u2) at (-5.5,-0.75){};
\node[noeud] (u3) at (-4,-0.75){};
\node[noeud] (u4) at (-4,-2.25){};
\node (u1') at (-5.3,-2.25){};
\node (u2') at (-5.3,-0.75){};
\node (u3') at (-3.8,-0.75){};
\node (u4') at (-3.8,-2.25){};

\node[right] at (u1){$u_1$};
\node[right] at (u2){$u_2$};
\node[right] at (u3){$u_3$};
\node[right] at (u4){$u_4$};

\draw \hedgeiii{u2'}{u3'}{u4'}{5mm};
\draw \hedgeii{u1'}{u2'}{5mm};
\draw \hedgeii{u1'}{u4'}{5mm};


\node[left] at (-5.7, -1.4){$A$};
\node[right] at (-3.4, -1){$C$};
\node at (-4.5, -2.9){$B$};

\end{tikzpicture}
}
\caption{Reduction from a hypergraph to a graph in the Domination game.}
\label{fig:Domination}
\end{figure}

==> hypergraph/pgf-hypergraph.tex <==
\def\hgrotate#1{
  % Rotate input point by 90 degrees counter-clockwise.
  \newdimen\x
  \pgfextractx{\x}{#1}
  \newdimen\y
  \pgfextracty{\y}{#1}
  \pgfpoint{-\y}{\x}
}

\def\hgperpr#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Compute a length-radius vector perpendicular (counter-clockwise)
  % to the line from start point to end point.
  \pgfpointscale{#3}{
    \hgrotate{
      \pgfpointnormalised{
        \pgfpointdiff{#1}{#2}}}}
}

\def\hgaddeperpr#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to end point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{#2}{\hgperpr{#1}{#2}{#3}}
}

\def\hgaddsperpr#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to start point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{\hgperpr{#1}{#2}{#3}}{#1}
}

\def\hgcorner#1#2#3#4{
  % #1 = previous point
  % #2 = current point
  % #3 = next point
  % #4 = radius
  % Draw a line to and a round corner on the outside of the angle #1#2#3.
  \pgflineto{\hgaddeperpr{#1}{#2}{#4}}
  \pgfmathanglebetweenpoints{#1}{#2}\let\anga\pgfmathresult
  % \pgfmathanglebetweenpoints{#2}{#3}\let\angb\pgfmathresult
  % \pgfpatharc{90 + \anga}{90 + \angb}{#4}
  \pgfpatharcto{#4}{#4}{90 + \anga}{0}{0}{\hgaddsperpr{#2}{#3}{#4}}
}

\def\hgedgeiiipriv#1#2#3#4{
  % #1#2#3 = pgf points
  % #4 = radius
  % Computes a path comprising the line of the points outside of the
  % convex hull H of the points #1#2#3 that have distance radius to H.
  % Points #1#2#3 need to be in clockwise order.
  \pgfpathmoveto{\hgaddeperpr{#3}{#1}{#4}}
  \hgcorner{#3}{#1}{#2}{#4}
  \hgcorner{#1}{#2}{#3}{#4}
  \hgcorner{#2}{#3}{#1}{#4}
  \pgfpathclose
}

\def\hgedgeiii#1#2#3#4{
  % #1#2#2 = pgf nodes
  % #4 = radius
  % Computes a path comprising the line of the points outside of the
  % convex hull H of the points #1#2#3 that have distance radius to H.
  % Points #1#2#3 need to be in clockwise order.
  \hgedgeiiipriv{
    \pgfpointanchor{#1}{center}}{
    \pgfpointanchor{#2}{center}}{
    \pgfpointanchor{#3}{center}}{
    #4}
}

\def\hgedgeiipriv#1#2#3{
  % #1#2 = pgf points
  % #3 = radius
  \pgfpathmoveto{\hgaddeperpr{#2}{#1}{#3}}
  \pgfpatharcto{#3}{#3}{90}{0}{0}{\hgaddsperpr{#1}{#2}{#3}}
  \pgflineto{\hgaddeperpr{#1}{#2}{#3}}
  \pgfpatharcto{#3}{#3}{270}{0}{0}{\hgaddsperpr{#2}{#1}{#3}}
  \pgfpathclose
}

\def\hgedgeii#1#2#3{
  \hgedgeiipriv{
    \pgfpointanchor{#1}{center}}{
    \pgfpointanchor{#2}{center}}{
    #3}
}


